Enhancing Multi-model Inference with Natural Selection

Multi-model inference covers a wide range of modern statistical applications such as variable selection, model confidence set, model averaging and variable importance. The performance of multi-model inference depends on the availability of candidate models, whose quality has been rarely studied in literature. In this paper, we study genetic algorithm (GA) in order to obtain high-quality candidate models. Inspired by the process of natural selection, GA performs genetic operations such as selection, crossover and mutation iteratively to update a collection of potential solutions (models) until convergence. The convergence properties are studied based on the Markov chain theory and used to design an adaptive termination criterion that vastly reduces the computational cost. In addition, a new schema theory is established to characterize how the current model set is improved through evolutionary process. Extensive numerical experiments are carried out to verify our theory and demonstrate the empirical power of GA, and new findings are obtained for two real data examples.

==> makefile <==
all:	PDFLaTeX Beamer clean

paper:	PDFLaTeX clean

slide:	Beamer clean

PDFLaTeX:	ga.tex
	pdflatex ga.tex
	bibtex ga
	pdflatex ga.tex
	pdflatex ga.tex

Beamer:	slide.tex
	pdflatex slide.tex
	bibtex slide
	perl -pi.bak -e 's/\\emph\{et~al.\}/\{\\em et~al.\}/g' slide.bbl
	pdflatex slide.tex
	pdflatex slide.tex

clean:	
	latexmk -c
	rm -f *.bbl *.nav *.snm *.bak

